Large-Scale Distributed Learning via Private On-Device Locality-Sensitive Hashing

Locality-sensitive hashing (LSH) based frameworks have been used efficiently to select weight vectors in a dense hidden layer with high cosine similarity to an input, enabling dynamic pruning. While this type of scheme has been shown to improve computational training efficiency, existing algorithms require repeated randomized projection of the full layer weight, which is impractical for computational- and memory-constrained devices. In a distributed setting, deferring LSH analysis to a centralized host is (i) slow if the device cluster is large and (ii) requires access to input data which is forbidden in a federated context. Using a new family of hash functions, we develop one of the first private, personalized, and memory-efficient on-device LSH frameworks. Our framework enables privacy and personalization by allowing each device to generate hash tables, without the help of a central host, using device-specific hashing hyper-parameters (e.g. number of hash tables or hash length). Hash tables are generated with a compressed set of the full weights, and can be serially generated and discarded if the process is memory-intensive. This allows devices to avoid maintaining (i) the fully-sized model and (ii) large amounts of hash tables in local memory for LSH analysis. We prove several statistical and sensitivity properties of our hash functions, and experimentally demonstrate that our framework is competitive in training large-scale recommender networks compared to other LSH frameworks which assume unrestricted on-device capacity.

==> Figures/Average-Neurons.tex <==
%\begin{figure*}[!t]
\centering
   %\begin{subfigure}[t]{0.45\textwidth}
   %\includegraphics[width=\textwidth]{Figures/Average-Neurons/Delicious200K-avg-neurons.pdf}
   %\caption{Delicious-200K Average Neurons per Sample.}
   %\label{fig:avg-neurons-del} 
%\end{subfigure}
%\begin{subfigure}[t]{0.45\textwidth}
   %\includegraphics[width=\textwidth]{Figures/Average-Neurons/Amazon670K-avg-neurons.pdf}
   %\caption{Amazon-670K Average Neurons per Sample.}
   %\label{fig:avg-neurons-amz}
%\end{subfigure}
\includegraphics[width=0.5\textwidth]{Figures/Average-Neurons/PGHash-avg-neurons.pdf}
\caption{\textbf{Average Activated Neurons.} We showcase that PGHash activates only a fraction of the total final layer neruons \textit{even without compression}. Through this induced sparsity, PGHash greatly reduces the computational complexity of forward and backward training compared to full training.}
\label{fig:avg-neurons}
%\end{figure*}

==> Figures/table-lsh.tex <==
\begin{table}[!htbp]
\caption{\textbf{Average LSH time for PGHash over a range of tables.} We compute the average $\mu$ time (and standard deviation $\sigma$) it takes for PGHash to perform \textit{vanilla sampling} (exact matches) between the hash codes of sample $x$ and each weight $w_i$ in the final dense layer. Times are sampled for PGHash on Delicious-200k for batch size $M=128$, $k=9$, and $c=8$ for one device.}
\centering
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Method} & \textbf{1 table (seconds)}        & \textbf{50 tables (seconds)}      & \textbf{100 tables (seconds)}     \\ \hline
PGHash          & $\mu=0.146$, $\sigma=0.009$ & $\mu=1.572$, $\sigma=0.045$ & $\mu=2.991$, $\sigma=0.041$ \\ \hline
SLIDE           & $\mu=0.147$, $\sigma=0.010$ & $\mu=1.593$, $\sigma=0.055$ & $\mu=2.999$, $\sigma=0.053$ \\ \hline
\end{tabular}
\label{tab:lsh-times}
\end{table}

==> extra.tex <==
the possible range of angles between a periodic Gaussian vector $s\in\mathbb{R}^d$ and an arbitrary $x\in\mathbb{R}^d$.
\begin{lemma}
\label{anglebound}
Fix $c<<d$ and assume $c|d$. Generate a random Gaussian vector $v\in\mathbb{R}^c$ with entries $[v]_i=s_i \sim \mathcal{N}(0,1)$ for $1\leq i \leq c$. Define a periodic Gaussian vector $v'$ with entries $[v']_i= s_{i \mod d/c}$ for $1\leq i \leq d$, which is a $c$-times repeated concatenation of $v$. Additionally, for any $x \in \mathbb{R}^d$, define $x_c\in \mathbb{R}^{c}$ as a bucketing of entries in $x$  with $[x_c]_j=\sum_{i=1}^{\frac{d}{c}}[x]_{j\cdot\frac{d}{c}+i}$ for $1\leq j \leq c$. We have then,
$|\cos(v',x)|\leq \sqrt{\frac{c}{d}}\frac{||x_c||_2}{||x||_2}$.
\end{lemma}
\begin{proof}
Notice that $v'^\top x =v^\top x_c$, which resembles the inner product between $c$-dimensional random Gaussian and an arbitrary $c$-dimensional vector. In particular, $\cos(v,x_c)$ is a continuous mapping onto $[-1,1]$ as we run over all such random Gaussian vectors $v$. Further, $||v'||_2=\sqrt{\frac{d}{c}}||v||_2$ since the entries of $v'$ periodically repeat $\frac{d}{c}$ times. Therefore, by definition of cosine similarity, $\cos(v',x)=\sqrt{\frac{c}{d}}\frac{||x_c||_2}{||x||_2}\cos(v,x_c)$, and our claim follows.
\end{proof}

Since $\frac{||x_c||_2}{||x||_2}\leq \sqrt{\frac{d}{c}}$ (each entry of $x_c$ is a bucketed sum of $\frac{d}{c}$ entries from $x$), the proof implies that for possible $v'$, the range of possible angles with a fixed $x$ is continuously mapped onto the interval $[\arccos(-\sqrt{\frac{c}{d}}\frac{||x_c||_2}{||x||_2}\cos(v,x_c),\sqrt{\frac{c}{d}}\frac{||x_c||_2}{||x||_2}\cos(v,x_c)]$ which is a compact subinterval centered about $\pi/2$ in $[0,\pi]$. This provides a great hint as to the sensitivity of $\mathcal{H}^{PG}$.
\begin{theorem}
\label{thm:pg-lsh}
    $\mathcal{H}^{PG}$ is LSH. 
\end{theorem}
\begin{proof}
We closely follow the argument of \cite[Lemma 3.2]{goemans1995improved}. Let $x,y\in \mathcal{R}^{d}$, i.e., the $d$-dimensional unit sphere, and let $v$ be a $d$-dimensional random Gaussian vector, and $c$ the chosen sketching dimension. Let $\alpha=\min\{\frac{||x_c||_2}{||x||_2},\frac{||y_c||_2}{||y||_2}\}$. We have by symmetry that $Pr(\textrm{sgn}(v^\top x)\neq \textrm{sgn}(v^\top y))=2 Pr(v^\top x \geq 0, v^\top y\leq 0 )$. The set $\{v^\top x \geq 0, v^\top y < 0 \}$ is the intersection of two half-spaces which form a dihedral angle of $\theta=\arccos(\cos(x,y))$. By Lemma \ref{anglebound}, its intersection with the periodic sphere (i.e., unit points with repeating entries) yields a spherical digon of angle $\hat{\theta}:=\arccos(\sqrt{\frac{c}{d}}\alpha\cos(\theta))$. By Lemma \ref{anglebound} and symmetry of the sphere, this set has measure $\frac{\hat{\theta}}{2\pi}$times the measure of the full sphere. Therefore, for a random $d$-dimensional periodic Gaussian vector $u$, $Pr(\textrm{sgn}(u^\top x)\neq \textrm{sgn}(u^\top y))=\frac{\hat{\theta}}{\pi}.$ Since $\hat{\theta}$ is monotonic with respect to the $\theta$, $\mathcal{H}^{PG}$ is LSH by Definition \ref{lsh-def}. 
\end{proof}

==> spare.tex <==
\begin{definition}[Correlated Gaussian Hash]
%\label{cgh}
Fix sketching dimension $c<<n$ and for simplicity, assume $c$ divides $n$. Let $B=[O_1\hspace{.1mm} | O_2 \hspace{.1mm} | \cdots\hspace{.1mm}| O_\frac{n}{c}]\in\mathbb{R}^{c\times n}$, where each $O_i \in \mathbb{R}^{c\times c}$ is an orthogonal matrix and $|$ denotes concatenation. Let $S\in\mathbb{R}^{c\times c}$ be a random Gaussian matrix with iid entries drawn from $\mathcal{N}(0,1)$. We may define a \textbf{correlated Gaussian hash} function $h_{B,S}: \mathbb{R}^d \rightarrow \mathbb{R}^c$ by $[h_{B,S}(x)]_i=[\textrm{sgn}(SBx)]_i$ for $1\leq i \leq c$. 
\end{definition}
We use the term "correlated" to describe the hash functions described in Definition \ref{cgh}, since the entries between two blocks $SO_i$ and $SO_j$ of $SB$ with $i\neq j$ are \textbf{dependent}. This follows from the well-known fact that orthogonal matrices of size $c\times c$ form a multiplicative group, i.e., there exists an invertible linear transformation $A\in\mathbb{R}^{c\times c}$ (namely, $O_i^{\top}O_j$) such that $SO_iA=SO_j$. However, the entries within each block are iid Gaussian drawn from $\mathcal{N}(0,1)$. 

Notice that we may easily extend the notion of a correlated Gaussian hash of one vector to an entire hash table over multiple vectors following Definition \ref{hashtable}. In this manner, we may generate a sequence of hash tables over a weight matrix $\{hB,S_i(W)\}_{i=1^K}$ simply by drawing a random Gaussian $S_i\in\mathbb{R}^{c\times c}$ and computing $\textrm{sgn}(S_iBW^\top)$. \textit{Hence, all a client needs access to is $BW^\top$, which is significantly cheaper to store.}

We observe that that the blocks $SO_i$ can never be decorrelated (at least not by a left matrix multiplication) as the base $B$ is conditioned on fixed orthogonal matrices. We argue then that there is no consequence to simply setting $B=[I_c\hspace{0.1mm}| I_c |\cdots | I_c] \in \mathbb{R}^{c\times n}$, where $I_c$ is the $c\times c$ identity matrix. 
